Spectral smooth tests for goodness-of-fit

Goodness-of-fit tests are crucial tools for assessing the validity of statistical models. In this paper, we introduce a novel approach, the Spectral Smooth Test (SST), that generalizes Neyman's smooth test to high-dimensional data settings. While conventional goodness-of-fit tests for univariate data are well-established, extending them to high dimensions, such as images, trajectories, and SNPs, poses significant challenges. Our proposed SST leverages spectral bases, which adapt naturally to the geometry of feature spaces, to model multivariate distributions. Unlike traditional orthogonal bases, these spectral bases are tailored to the data distribution, enabling more effective function modeling. The SST framework offers a principled way to estimate the underlying model, thereby providing actionable insights even when the null hypothesis is rejected. We present experimental results demonstrating the robustness of SST across various tuning parameter choices and compare its performance against other goodness-of-fit tests. Furthermore, we apply SST to the MNIST dataset as a real-world example, showcasing its effectiveness in high-dimensional scenarios.

==> algorithms.tex <==

\vspace{0.5cm}

In the sequence we listed algorithms to apply the SST test.

\begin{algorithm}[!ht]
	\caption{
	%Estimate
	Estimate $|\Lambda|$ distributions under $H_0$
	%coverage.
	}\label{alg:pdist}
	\algorithmicrequire \ {\small  Bandwidths, thresholds.
}\\
	\algorithmicensure \ {\small $|\Lambda|$ distributions of $T_{\lambda}$ under $H_0$}
	\begin{algorithmic}[1]
	
	\State Simulate $C_1$ the set of $H_0$ samples for estimate sets of $\{\theta_i\}$'s
    \State \For {\textbf{each} element in $C_1$}

    \State	\For {\textbf{each} pair of bandwidth and threshold indexed by $\lambda \in \Lambda$}
	
	\State Perform the algorithm \ref{alg:eigenf} 
 
	\State Calculate kernels between target sample and $H_0$ sample for basis

    \State Calculate $\widehat{\psi}_i(.)$ (Equation \ref{eq:expsi})

	\State Calculate $s(.)$ for each element of $H_0$ basis sample

	\State	Combine the previous results to get
	$\widehat{\theta_i}$(Equation \ref{eq:estimated_theta})
	\EndFor
	
	\State	\For {\textbf{each} pair of bandwidth and threshold indexed by $\lambda \in \Lambda$}
	\State Compute $T_{\lambda}$ (Equation \ref{eq:test_one})
    \EndFor
	\EndFor    
    \State \textbf{return} $|\Lambda|$ distributions of $T_{\lambda}$ under $H_0$
	\end{algorithmic}
\end{algorithm}




\begin{algorithm}[!ht]
	\caption{
	%Estimate
	Statistic for a sample
	%coverage.
	}\label{alg:stat}
	\algorithmicrequire \ {\small Bandwidths, thresholds, target sample.
}\\
	\algorithmicensure \ {\small A single statistic $T_{SST}$ from target sample}
	\begin{algorithmic}[1]

    \State Perform the algorithm \ref{alg:pdist}

    \State \For {each bandwidth and threshold indexed by $\lambda$}

        \State 	Calculate $T_{\lambda}^*$ (Equation \ref{eq:rtl}) for the target sample and $p_k$
    \EndFor
        \State Compute a statistic $T_{SST}$ (Equation \ref{eq:statistic})
        \State \textbf{return} $T_{SST}$
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[!ht]
	\caption{
	%Estimate
	Final distribution
	%coverage.
	}\label{alg:dist}
	\algorithmicrequire \ {\small Bandwidths, thresholds.}\\
	\algorithmicensure \ {\small Final distribution}
	\begin{algorithmic}[1]

    
    \State Simulate $C_2$ the set of $H_0$ samples to estimate the final distribution
    
        \State 	\For{\textbf{each} element in $C_2$}

        \State Perform algorithm \ref{alg:stat} 
    \EndFor

    \State \textbf{return} Final distribution
	\end{algorithmic}
\end{algorithm}


